Breaking electron pairs in the pseudogap regime of SmTiO$_3$/SrTiO$_3$/SmTiO$_3$ quantum wells

The strongly correlated two-dimensional electron liquid within SmTiO$_3$/SrTiO$_3$/SmTiO$_3$ quantum well structures exhibits a pseudogap phase when the quantum well width is sufficiently narrow. Using low-temperature transport and optical experiments that drive the quantum-well system out of equilibrium, we find evidence of mobile, long-lived, negatively-charged quasiparticles, consistent with the idea that the pseudogap phase arises from strongly bound electron pairs.

==> errors.tex <==
Cornell University
We gratefully acknowledge support from
the Simons Foundation and member institutions.
arxiv logo
> submitLogged in as jlevy | Help | My Account | Logout
Start   >>   Add Files   >>   Process   >>   Metadata   >>   Preview

Submission Processing
Reprocess


arXiv's automated TeX processing has failed to process your source. The 5 most common mistakes causing this are:

1. Mixed figure file formats. If you are using PDFLaTeX then all figures must be .pdf, .jpg, or .png formats. If your document uses (La)TeX all figures must be .ps or .eps. arXiv does not perform figure file conversion for you, please ensure your files are converted to the appropriate format before uploading.
2. File-name upper/lower-case mismatch between TeX source and figure or included files. arXiv's file system is case sensitive.
3. Default hyperref failures ("Option clash for package hyperref") are not a reason to report a failure to arXiv. Continue scrolling in the log to find the specific errors that are being flagged.
4. Missing customized or differing version of style files.
5. Missing, misnamed, or local complete paths to figure files. arXiv's file system is case sensitive.

The TeX Log appears below. If you are unsure of what your specific failure is and cannot resolve the issue after reviewing our help pages, or searching the internet for your specific errors, please contact us citing submit/4876121 to ensure a more rapid response. Please note that it may take a day or two to receive a personal response.

You may wish to hit "Ctrl + F" ("Apple + F" on a Mac) or browse to Edit and select "Find" to search for "error". Please note that the first error may simply be arXiv's application of hypertex failing.


Processing Status: Failed

If you are attempting to compile with a specific engine (PDFLaTeX, LaTeX,
TeX) please carefully review the appropriate log below.

Summary of attempted TeX compilation runs:

  Processing;'main.tex'
    Running pdflatex for first time.
    Running tex for first time.

  Last run per file and engine
    main.tex:
      Last run for engine pdflatex is first
      Last run for engine tex is first

Key for Highlighted AutoTeX Log:
Severe warnings/errors.'
Warnings deemed important'
General warnings/errors from packages.'
Warnings/Errors deemed unimportant. Example: undefined references in first TeX run.'
Indicates positive event, does not guarantee overall success
Informational markup
References to arXiv help pages or other documentation.
Highlighted AutoTeX Log:

[verbose]: Creating arXiv submission AutoTeX object
[verbose]: *** Using TeX Live 2020 ***
[verbose]: Calling arXiv submission AutoTeX process
[verbose]: TeX/AutoTeX.pm: admin_timeout = minion
[verbose]: <SmTO_V3_Fig_3.pdf> is of type 'PDF'.
[verbose]: <Fig_1_R1.pdf> is of type 'PDF'.
[verbose]: <Fig_3.pdf> is of type 'PDF'.
[verbose]: <SmTO_V3_Fig_4.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <SmTO_V3_Fig_5.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <SmTO_V3_Fig_6.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <SmTO_V3_Fig_7.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <SmTO_V4_Fig_1.pdf> is of type 'PDF'.
[verbose]: <SmTO_V4_Fig_5.pdf> is of type 'PDF'.
[verbose]: <SmTO_V4_Fig_ac.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <SmTO_optical.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <fig4.png> is of type 'Image (gif/jpg etc)'.
[verbose]: <main.bbl> is of type 'TeX auxiliary'.
[verbose]: <main.tex> is of type 'PDFLATEX'.
[verbose]: <paperpile.bib> is of type 'BiBTeX'.
[verbose]: ~~~~~~~~~~~ Processing file 'main.tex'
[verbose]: arXiv Warning: user included plain hyperref directive.
[verbose]: TEXMFCNF is unset.
[verbose]: ~~~~~~~~~~~ Running pdflatex for the first time ~~~~~~~~
[verbose]: Running: "(export HOME=/tmp PATH=/texlive/2020/bin/arch:/bin; cd /submissions/4876121/ && pdflatex 'main.tex' < /dev/null)" 2>&1
[verbose]: This is pdfTeX, Version 3.14159265-2.6-1.40.21 (TeX Live 2020) (preloaded format=pdflatex)
restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2020-02-02> patch level 5
L3 programming layer <2020-09-06>
(/texlive/2020/texmf-dist/tex/latex/revtex/revtex4-2.cls
Document Class: revtex4-2 2019/01/18/14:29:48 4.2c (https://journals.aps.org/re
vtex/ for documentation)
ltxutil[2019/01/18/14:29:48 4.2c utilities package (portions licensed from W. E
. Baxter web at superscript.com)]
ltxfront[2019/01/18/14:29:48 4.2c frontmatter package (AO,DPC,MD)]
ltxgrid[2019/01/18/14:29:48 4.2c page grid package (portions licensed from W. E
. Baxter web at superscript.com)]

Class revtex4-2 Warning: Failed to recognize \@vspace, \@vspacer, \@no@pgbk, \@
newline, and \\; no patches applied. Please get a more up-to-date class, .

(/texlive/2020/texmf-dist/tex/latex/revtex/aps4-2.rtx)

Class revtex4-2 Warning: No journal specified, using default pra.

(/texlive/2020/texmf-dist/tex/latex/revtex/aps10pt4-2.rtx)
(/texlive/2020/texmf-dist/tex/latex/textcase/textcase.sty)
(/texlive/2020/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/texlive/2020/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/texlive/2020/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/texlive/2020/texmf-dist/tex/latex/amsmath/amstext.sty
(/texlive/2020/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/texlive/2020/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/texlive/2020/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/texlive/2020/texmf-dist/tex/latex/url/url.sty)
(/texlive/2020/texmf-dist/tex/latex/natbib/natbib.sty)
(/texlive/2020/texmf-dist/tex/latex/revtex/revsymb4-2.sty))
(/texlive/2020/texmf-dist/tex/latex/graphics/graphicx.sty
(/texlive/2020/texmf-dist/tex/latex/graphics/keyval.sty)
(/texlive/2020/texmf-dist/tex/latex/graphics/graphics.sty
(/texlive/2020/texmf-dist/tex/latex/graphics/trig.sty)
(/texlive/2020/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/texlive/2020/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/texlive/2020/texmf-dist/tex/latex/tools/dcolumn.sty
(/texlive/2020/texmf-dist/tex/latex/tools/array.sty))
(/texlive/2020/texmf-dist/tex/latex/tools/bm.sty)
(/texlive/2020/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def)
No file main.aux.
(/texlive/2020/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/texlive/2020/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/texlive/2020/texmf-config/tex/latex/latexconfig/epstopdf-sys.cfg))
(/texlive/2020/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/texlive/2020/texmf-dist/tex/latex/amsfonts/umsb.fd)

Package natbib Warning: Citation `Ding1996-vm' on page 1 undefined on input lin
e 85.


Package natbib Warning: Citation `Loeser1996-jo' on page 1 undefined on input l
ine 85.


Package natbib Warning: Citation `Timusk1999-pr' on page 1 undefined on input l
ine 85.


Package natbib Warning: Citation `Lee2006-os' on page 1 undefined on input line
85.


Package natbib Warning: Citation `Shimojima2014-qt' on page 1 undefined on inpu
t line 85.


Package natbib Warning: Citation `Tohyama2011-bf' on page 1 undefined on input
line 87.


Package natbib Warning: Citation `Sidorov2002-pi' on page 1 undefined on input
line 87.


Package natbib Warning: Citation `Rossnagel2011-ad' on page 1 undefined on inpu
t line 87.


Package natbib Warning: Citation `Allen2015-zr' on page 1 undefined on input li
ne 87.


Package natbib Warning: Citation `Stewart2008-zj' on page 1 undefined on input
line 87.


Package natbib Warning: Citation `Jochim2003-bz' on page 1 undefined on input l
ine 87.


Package natbib Warning: Citation `Richter2013-lr' on page 1 undefined on input
line 87.


Package natbib Warning: Citation `Marshall2015-cv' on page 1 undefined on input
line 87.


Package natbib Warning: Citation `Bozovic2020-tt' on page 1 undefined on input
line 89.


Package natbib Warning: Citation `Randeria2014-fz' on page 1 undefined on input
line 89.


Package natbib Warning: Citation `He2011-qj' on page 1 undefined on input line
89.


Package natbib Warning: Citation `Schooley1964-xx' on page 1 undefined on input
line 93.


Package natbib Warning: Citation `Koonce1967-sl' on page 1 undefined on input l
ine 93.


Package natbib Warning: Citation `Pai2018-br' on page 1 undefined on input line
93.


Package natbib Warning: Citation `Reyren2007-sz' on page 1 undefined on input l
ine 93.


Package natbib Warning: Citation `Caviglia2008-bf' on page 1 undefined on input
line 93.


Package natbib Warning: Citation `Richter2013-lr' on page 1 undefined on input
line 93.


Package natbib Warning: Citation `Cheng2015-fv' on page 1 undefined on input li
ne 93.


Package natbib Warning: Citation `Prawiroatmodjo2017-ke' on page 1 undefined on
input line 93.


Package natbib Warning: Citation `Annadi2018-az' on page 1 undefined on input l
ine 93.


Package natbib Warning: Citation `Briggeman2020-cl' on page 1 undefined on inpu
t line 93.


Package natbib Warning: Citation `Jackson2013-bo' on page 1 undefined on input
line 109.


Package natbib Warning: Citation `Moetakef2012-sr' on page 1 undefined on input
line 109.


Package natbib Warning: Citation `Zhang2014-qy' on page 1 undefined on input li
ne 109.


Package natbib Warning: Citation `Mikheev2015-yw' on page 1 undefined on input
line 109.


Package natbib Warning: Citation `Mikheev2015-yw' on page 1 undefined on input
line 109.


Package natbib Warning: Citation `Jackson2014-tm' on page 1 undefined on input
line 111.


Package natbib Warning: Citation `Stemmer2018-hj' on page 1 undefined on input
line 111.


Package natbib Warning: Citation `Marshall2016-jd' on page 1 undefined on input
line 113.


Package natbib Warning: Citation `Ahadi2017-hq' on page 1 undefined on input li
ne 113.


Package natbib Warning: Citation `Joshua2012-vy' on page 1 undefined on input l
ine 113.


LaTeX Warning: File `SmTO V4 Fig 5.pdf' not found on input line 117.


! Package pdftex.def Error: File `SmTO V4 Fig 5.pdf' not found: using draft set
ting.

See the pdftex.def package documentation for explanation.
Type H <return> for immediate help.
...

l.117 ...egraphics[width=5.5cm]{SmTO V4 Fig 5.pdf}
% Here is how to import EP...

?
! Emergency stop.
...

l.117 ...egraphics[width=5.5cm]{SmTO V4 Fig 5.pdf}
% Here is how to import EP...

! ==> Fatal error occurred, no output PDF file produced!
Transcript written on main.log.

[verbose]: pdflatex 'main.tex' failed.
[verbose]: Removing (La)TeX AUX file called 'main.aux' (1683171238 >= 1683171237)
[verbose]: Removing (La)TeX AUX file called 'mainNotes.bib' (1683171238 >= 1683171237)
[verbose]: 'htex' is not a valid TeX format; will ignore.
[verbose]: TEXMFCNF is unset.
[verbose]: ~~~~~~~~~~~ Running tex for the first time ~~~~~~~~
[verbose]: Running: "(export HOME=/tmp PATH=/texlive/2020/bin/arch:/bin; cd /submissions/4876121/ && tex 'main.tex' < /dev/null)" 2>&1
[verbose]: This is TeX, Version 3.14159265 (TeX Live 2020) (preloaded format=tex)
(./main.tex
! Undefined control sequence.
l.1 \documentclass
[floatfix,
?
! Emergency stop.
l.1 \documentclass
[floatfix,
No pages of output.
Transcript written on main.log.

[verbose]: tex 'main.tex' failed.
[verbose]: We failed utterly to process the TeX file 'main.tex'
[error]: Unable to sucessfully process tex files.
*** AutoTeX ABORTING ***

[verbose]: AutoTeX returned error: Unable to sucessfully process tex files.

[verbose]: $autotex->process failed $@: $?: 0 $!: Inappropriate ioctl for device
[verbose]: Error running AutoTeX process:


About
Help
Contact
Subscribe
Copyright
Privacy Policy
Web Accessibility Assistance
arXiv Operational Status 
Get status notifications via email or slack
